Sonnet or Not, Bot? Poetry Evaluation for Large Models and Datasets

Large language models (LLMs) can now generate and recognize poetry. But what do LLMs really know about poetry? We develop a task to evaluate how well LLMs recognize one aspect of English-language poetry--poetic form--which captures many different poetic features, including rhyme scheme, meter, and word or line repetition. By using a benchmark dataset of over 4.1k human expert-annotated poems, we show that state-of-the-art LLMs can successfully identify both common and uncommon fixed poetic forms--such as sonnets, sestinas, and pantoums--with surprisingly high accuracy. However, performance varies significantly by poetic form; the models struggle to identify unfixed poetic forms, especially those based on topic or visual features. We additionally measure how many poems from our benchmark dataset are present in popular pretraining datasets or memorized by GPT-4, finding that pretraining presence and memorization may improve performance on this task, but results are inconclusive. We release a benchmark evaluation dataset with 1.4k public domain poems and form annotations, results of memorization experiments and data audits, and code.

==> latex/tables/fixed_forms_not_dolma_performance.tex <==
\begin{table*}[t]
    \scriptsize
    \centering
    \begin{tabular}{lcccccccccccccccccccc}
    \toprule
    & \multicolumn{3}{c}{Sonnet} & \multicolumn{3}{c}{Limerick} & \multicolumn{3}{c}{Haiku} & \multicolumn{3}{c}{Ballad} \\\cmidrule(lr){2-4}\cmidrule(lr){5-7}\cmidrule(lr){8-10}\cmidrule(lr){11-13}
               model & f1 & precision & recall & f1 & precision & recall & f1 & precision & recall & f1 & precision & recall \\\midrule
    GPT-3.5 & \gradient{0.91} & 0.92 & 0.91 & \gradient{1.00} & 1.00 & 1.00 & \gradient{0.89} & 0.90 & 0.88 & \gradient{0.78} & 0.82 & 0.75 \\
    GPT-4   & \gradient{0.94} & 0.98 & 0.90 & \gradient{0.89} & 0.80 & 1.00 & \gradient{1.00} & 1.00 & 1.00 & \gradient{0.87} & 0.85 & 0.89 \\
    GPT-4o  & \gradient{0.94} & 0.99 & 0.89 & \gradient{1.00} & 1.00 & 1.00 & \gradient{0.90} & 0.96 & 0.84 & \gradient{0.90} & 0.93 & 0.88 \\
    Claude  & \gradient{0.94} & 0.94 & 0.95 & \gradient{0.80} & 0.67 & 1.00 & \gradient{0.93} & 1.00 & 0.88 & \gradient{0.79} & 0.98 & 0.67 \\
    Mixtral & \gradient{0.92} & 0.95 & 0.88 & \gradient{0.89} & 0.80 & 1.00 & \gradient{0.84} & 0.96 & 0.75 & \gradient{0.76} & 0.73 & 0.79 \\
    Llama3  & \gradient{0.74} & 1.00 & 0.58 & \gradient{0.67} & 0.50 & 1.00 & \gradient{0.84} & 0.96 & 0.75 & \gradient{0.49} & 0.35 & 0.82 \\\midrule
    & \multicolumn{3}{c}{Sestina} & \multicolumn{3}{c}{Villanelle} & \multicolumn{3}{c}{Pantoum} & \multicolumn{3}{c}{Ghazal} \\\cmidrule(lr){2-4}\cmidrule(lr){5-7}\cmidrule(lr){8-10}\cmidrule(lr){11-13}
               model & f1 & precision & recall & f1 & precision & recall & f1 & precision & recall & f1 & precision & recall \\\midrule
    GPT-3.5 & \gradient{0.08} & 1.00 & 0.04 & \gradient{0.65} & 0.49 & 0.94 & \gradient{0.33} & 0.75 & 0.21 & \gradient{0.47} & 0.40 & 0.57 \\
    GPT-4   & \gradient{0.84} & 0.84 & 0.84 & \gradient{0.91} & 0.97 & 0.85 & \gradient{0.80} & 0.67 & 1.00 & \gradient{0.68} & 0.53 & 0.95 \\
    GPT-4o  & \gradient{0.77} & 0.69 & 0.88 & \gradient{0.93} & 0.89 & 0.97 & \gradient{0.82} & 0.70 & 1.00 & \gradient{0.50} & 0.35 & 0.90 \\
    Claude  & \gradient{0.38} & 0.30 & 0.52 & \gradient{0.56} & 0.54 & 0.59 & \gradient{0.59} & 0.62 & 0.57 & \gradient{0.49} & 0.50 & 0.48 \\
    Mixtral & \gradient{0.21} & 1.00 & 0.12 & \gradient{0.79} & 0.96 & 0.68 & \gradient{0.67} & 0.55 & 0.86 & \gradient{0.64} & 0.58 & 0.71 \\
    Llama3  & \gradient{0.14} & 0.67 & 0.08 & \gradient{0.31} & 0.19 & 0.88 & \gradient{0.59} & 0.44 & 0.86 & \gradient{0.25} & 0.36 & 0.19 \\\bottomrule
    \end{tabular}
    \caption{\textbf{Fixed Forms — Detection With Only Poem Text — Not Found in Dolma.} This table shows LLM performance by model on the task of detecting poetic form (in the same way as the human annotation/institution it was collected from) when the model is prompted only with the text of the poem.}
    \label{table:evaluation-results}
\end{table*}


==> latex/tables/fixed_forms_performance_all_shaded.tex <==
\begin{table*}[t]
    \scriptsize
    \centering
    \begin{tabular}
    {lcccccccccccccccccc}
    \toprule
    & \multicolumn{3}{c}{Sonnet} & \multicolumn{3}{c}{Limerick} & \multicolumn{3}{c}{Haiku} & \multicolumn{3}{c}{Ballad} \\\cmidrule(lr){2-4}\cmidrule(lr){5-7}\cmidrule(lr){8-10}\cmidrule(lr){11-13}
               model & f1 & precision & recall & f1 & precision & recall & f1 & precision & recall & f1 & precision & recall \\\midrule
    GPT-3.5 & \gradient{0.92} & \gradient{0.98} & \gradient{0.86} & \gradient{0.78} & \gradient{0.64} & \gradient{1.00} & \gradient{0.93} & \gradient{0.91} & \gradient{0.96} & \gradient{0.77} & \gradient{0.74} & \gradient{0.80} \\
    GPT-4   & \gradient{0.94} & \gradient{0.98} & \gradient{0.91} & \gradient{0.82} & \gradient{0.70} & \gradient{1.00} & \gradient{0.94} & \gradient{0.93} & \gradient{0.96} & \gradient{0.85} & \gradient{0.82} & \gradient{0.88} \\
    GPT-4o  & \gradient{0.93} & \gradient{0.99} & \gradient{0.87} & \gradient{1.00} & \gradient{1.00} & \gradient{1.00} & \gradient{0.94} & \gradient{0.94} & \gradient{0.94} & \gradient{0.85} & \gradient{0.84} & \gradient{0.87} \\
    Claude  & \gradient{0.95} & \gradient{0.97} & \gradient{0.94} & \gradient{0.88} & \gradient{0.78} & \gradient{1.00} & \gradient{0.90} & \gradient{0.96} & \gradient{0.85} & \gradient{0.80} & \gradient{0.93} & \gradient{0.71} \\
    Mixtral & \gradient{0.92} & \gradient{0.95} & \gradient{0.90} & \gradient{0.88} & \gradient{0.78} & \gradient{1.00} & \gradient{0.80} & \gradient{0.95} & \gradient{0.69} & \gradient{0.73} & \gradient{0.68} & \gradient{0.79} \\\midrule
    & \multicolumn{3}{c}{Sestina} & \multicolumn{3}{c}{Villanelle} & \multicolumn{3}{c}{Pantoum} & \multicolumn{3}{c}{Ghazal} \\\cmidrule(lr){2-4}\cmidrule(lr){5-7}\cmidrule(lr){8-10}\cmidrule(lr){11-13}
               model & f1 & precision & recall & f1 & precision & recall & f1 & precision & recall & f1 & precision & recall \\\midrule
    GPT-3.5 & \gradient{0.15} & \gradient{0.67} & \gradient{0.09} & \gradient{0.55} & \gradient{0.38} & \gradient{0.99} & \gradient{0.32} & \gradient{0.83} & \gradient{0.20} & \gradient{0.58} & \gradient{0.46} & \gradient{0.79} \\
    GPT-4   & \gradient{0.78} & \gradient{0.76} & \gradient{0.80} & \gradient{0.95} & \gradient{0.98} & \gradient{0.91} & \gradient{0.83} & \gradient{0.73} & \gradient{0.96} & \gradient{0.74} & \gradient{0.63} & \gradient{0.91} \\
    GPT-4o  & \gradient{0.72} & \gradient{0.62} & \gradient{0.87} & \gradient{0.88} & \gradient{0.82} & \gradient{0.96} & \gradient{0.86} & \gradient{0.77} & \gradient{0.96} & \gradient{0.61} & \gradient{0.47} & \gradient{0.88} \\
    Claude  & \gradient{0.44} & \gradient{0.33} & \gradient{0.67} & \gradient{0.63} & \gradient{0.62} & \gradient{0.64} & \gradient{0.49} & \gradient{0.55} & \gradient{0.44} & \gradient{0.45} & \gradient{0.43} & \gradient{0.47} \\
    Mixtral & \gradient{0.23} & \gradient{0.86} & \gradient{0.13} & \gradient{0.63} & \gradient{0.60} & \gradient{0.67} & \gradient{0.33} & \gradient{0.41} & \gradient{0.28} & \gradient{0.61} & \gradient{0.76} & \gradient{0.51} \\\bottomrule
    \end{tabular}
    \caption{LLM Evaluation of \textbf{Fixed Forms} (When Prompted With Text Only)}
    \label{table:evaluation-results}
\end{table*}
